Entropy-Based Adaptive Weighting for Self-Training

The mathematical problem-solving capabilities of large language models have become a focal point of research, with growing interests in leveraging self-generated reasoning paths as a promising way to refine and enhance these models. These paths capture step-by-step logical processes while requiring only the correct answer for supervision. The self-training method has been shown to be effective in reasoning tasks while eliminating the need for external models and manual annotations. However, optimizing the use of self-generated data for model training remains an open challenge. In this work, we propose Entropy-Based Adaptive Weighting for Self-Training (EAST), an adaptive weighting strategy designed to prioritize uncertain data during self-training. Specifically, EAST employs a mapping function with a tunable parameter that controls the sharpness of the weighting, assigning higher weights to data where the model exhibits greater uncertainty. This approach guides the model to focus on more informative and challenging examples, thereby enhancing its reasoning ability. We evaluate our approach on GSM8K and MATH benchmarks. Empirical results show that, while the vanilla method yields virtually no improvement (0%) on MATH, EAST achieves around a 1% gain over backbone model. On GSM8K, EAST attains a further 1-2% performance boost compared to the vanilla method.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/exp2.tex <==

\section{Experiment}

In this section, we present the experiment setting in Section~\ref{sec:setting} and provide main result in Section~\ref{sec:result}. Then, we provide further in-depth discussion and ablation study in Section~\ref{sec:ablation}. 
\subsection{Experiment Setting}
\label{sec:setting}
\textbf{Model Configuration}
% We conduct the experiment under two backbone model: Llama-3.2-1B-Instruct and Llama-3.1-8B-Instruct. For SFT, we use learning rate of 1e-6 for both model; for DPO, we adopt learning rate of 1e-7. Each model is trained for three epochs with a batch size of 16. We set $\alpha$=0.5 for both methods. We adapt $a_H, b_H, t_H$ as 0.39, 0, 0 for GSM8k and 0.33,0,0.1 for MATH; $a_A, b_A, t_A$ as 0.19,0,0 for GSM8k and 2,0.6,0 for MATH. 
We conduct the experiment using two backbone models: Llama-3.2-1B-Instruct and Llama-3.1-8B-Instruct. For SFT, we use a learning rate of $1e^{-6}$ for both models; for DPO, we adopt a learning rate of $1e^{-7}$. Each model is trained for three epochs with a batch size of 16. We set $\alpha$ = 0.5 for both methods. We adapt the entropy-based weighting parameters $(a_H, b_H, t_H)$ as $(0.39, 0, 0)$ for GSM8K and $(0.33, 0, 0.1)$ for MATH. Similarly, we set the accuracy-based weighting parameters $(a_A, b_A, t_A)$ as $(0.19, 0, 0)$ for GSM8K and $(2, 0.6, 0)$ for MATH.
\\\\
\textbf{Dataset}
% We adapt two mathematical benchmark: MATH~\citep{hendrycks2021measuring} and GSM8K~\citep{cobbe2021training}. The MATH dataset comprises 7k5 for training data and 5k problems for test data, covering a range of mathematical domains, including algebra, geometry, probability, number theory, and calculus. The GSM8K test set contains 7.47k problems for training data and 1,31k for test data grade-school-level math word problems, which are generally simpler than those in MATH. For training data, we prompot backbone model with training questions and geenralte 128 samples for each question. For evaluation, we use vllm with temperature of 0 and adapt the evaluation piepline of \citet{yang2024qwen2}. 
We adapt two mathematical benchmarks: MATH~\citep{hendrycks2021measuring} and GSM8K~\citep{cobbe2021training}. The MATH dataset comprises 7.5k training problems and 5k test problems, covering a range of mathematical domains, including algebra, geometry, probability, number theory, and calculus. The GSM8K dataset contains 7.47k training problems and 1.31k test problems, consisting of grade-school-level math word problems, which are generally simpler than those in MATH. 

For training, we prompt the backbone model with training questions and generate 128 samples for each question. For evaluation, we use vLLM with a temperature of 0 and adapt the evaluation pipeline of \citet{yang2024qwen2}.
\\\\
\textbf{Baseline}
We compare our approach with other alignment methods: KTO~\citep{ethayarajh2024kto} optimizes generation utility using unpaired data rather than focusing on maximizing the log-likelihood of preferences. ORPO~\citep{hong2024orpo} leverages a reference-model-free odds ratio term to contrast winning and losing responses while jointly optimizing with the SFT objective. SimPO~\citep{meng2024simpo} optimizes preferences by aligning rewards with generation metrics using a length-normalized reward and a target reward margin. WPO~\citep{zhou2024wpo}, which weights preference pairs to mitigate distribution mismatch.


\subsection{Experiment Results}
\label{sec:result}
As shown in Table~\ref{table:main}, while all evaluated methods improve upon the default model, APO surpasses all baselines on both datasets, achieving an overall AVG of 40.31$\%$. Among preference optimization methods, WPO and DPO achieve strong results, with WPO reaching 39.51$\%$ and DPO 39.32$\%$. Notably, APO attains an accuracy of 50.80$\%$ on GSM8K, outperforming WPO of 49.66$\%$, and an accuracy of 29.82$\%$ on MATH, compared to vanilla DPO of 29.36$\%$ and SFT 27.82$\%$. These results highlight the effectiveness of APO in advancing mathematical reasoning performance.
\input{apo/table/main_exp}
\subsection{Ablation and Discussion}
\label{sec:ablation}
\input{apo/table/ablation}
\subsubsection*{The comparison between Accuracy-based weight and Entropy-based weight and the corresponding reverse weight for them. }
% \label{sec:ablation}
To further demonstrate the effectiveness of our method, we investigate both accuracy-based and entropy-based weighting schemes, as well as their reversed variants. Let \(w \in [0,1]\) denote the original weight for a training example, where the average value of \(w\) is constrained to 1 across all training data. We define the reversed weight as:
% \begin{equation}
    $w_{\mathrm{rev}} = 2 - w$,
% \end{equation}
which ensures symmetry around 1. 

As reported in Table~\ref{table:ablation}, both accuracy-based and entropy-based weights exhibit monotonic improvements. In particular, the accuracy-based approach increases the GSM8K score from 48.90$\%$ to 50.57$\%$ and the MATH score from 29.20$\%$ to 30.28$\%$. These results confirm that our proposed weighting component consistently enhances model training performance.
\subsubsection*{Effect of Reject-Dominant Weights}

Recent studies indicate that large language models (LLMs) struggle with self-correction, particularly when they generate responses with high confidence~\citep{kumar2024training, yang2024confidence}. To further investigate this phenomenon, we propose a novel weighting scheme that prioritizes the most “stubborn” questions—those for which the model repeatedly produces the same incorrect answers.

Specifically, for all samples that yield incorrect answers, we partition them into $\hat{k}$ clusters, where each cluster corresponds to a distinct final answer. We assume that samples leading to the same (incorrect) answer follow similar reasoning patterns. Next, we calculate the proportion of each incorrect answer cluster and identify the most frequent (dominant) mistake. The weight of this question is assigned based to the portion of this dominant mistake through a linear transformation, as detailed in Section~\ref{sec:acc}.

The empirical findings, presented in Table~\ref{table:ablation}, indicate that applying the dominant-reject weighting scheme leads to a decline in performance, with an average accuracy of 38.91$\%$ across two benchmarks, compared to 40.15$\%$ achieved using the Accuracy-Based weighting scheme. This outcome suggests that prioritizing “stubborn” questions—those that consistently result in a common erroneous answer—does not offer benefits for model training. 
\subsubsection*{The comparison between different algorithm using APO}
\input{apo/table/ablation_sft}
Besides DPO, SFT and other alignment methods are frequently adopted in self-training pipelines. Because APO operates by reweighting self-generated data and does not depend on any particular loss function, it can be seamlessly integrated with these methods. To assess whether APO improves performance across different losses, we consider two representative approaches: SFT, which relies exclusively on positive samples, and KTO, which utilizes unpaired data. In both cases, we assign prompt-specific weights such that the average weight in the training set is 1. As shown in Table~\ref{table:sft}, incorporating APO yields consistent improvements for both SFT and KTO, especially for SFT, which increases from 27.82$\%$ to 29.00$\%$ on the MATH dataset. This suggests that APO provides a general performance boost across diverse self-training and alignment methods.
% \subsubsection*{Iterative training of DPO and APO?}

\subsubsection*{The impact of threshold on Accuracy-Based and Entropy-Based Weights}
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=\linewidth]{figure/threshold.pdf}
% 	\caption{Results of applying different thresholds on Accuracy-based and Entropy-based weights.}
% 	\label{fig:t}
%  \vskip-0.5em
% \end{figure}
When a dataset contains problems spanning a wide range of difficulty, simply assigning higher weights or attention to the most challenging questions does not necessarily lead to better performance. This observation aligns with educational theories suggesting that learners benefit more from tasks within their “zone of proximal development,” meaning tasks that are neither trivial nor overwhelmingly difficult~\citep{vygotsky1977development}. Extremely difficult problems, in particular, may encourage rote memorization rather than deeper reasoning.

To investigate the impact of heavily reweighting the most error-prone items, we introduce a threshold on the accuracy rate. Specifically, any problem with an accuracy below this threshold is assigned a fixed weight (e.g. w=1). As illustrated in Figure~\ref{fig:t}, applying this threshold leads to a decline in performance on GSM8K, suggesting that for relatively easier datasets, prioritizing the most challenging yet solvable problems can be beneficial. Conversely, down-weighting these problems adversely affects overall learning.

In contrast, for the MATH benchmark under entropy-based weighting, we observe a performance improvement when applying a threshold of 0.05. This finding suggests that problems with accuracy rates below 0.05—representing extremely difficult or highly error-prone cases—may contribute little to learning progress. Instead, moderately challenging problems appear to be more effective for skill acquisition. Notably, this trend does not emerge under accuracy-based weighting, highlighting the sensitivity of the relationship between problem difficulty, uncertainty, and performance to the specific weighting criterion employed.


==> section/intro2.tex <==
To address this gap, we introduce \textbf{E}ntropy-Based \textbf{A}daptive Weighting for \textbf{S}elf-\textbf{T}raining (EAST), a novel method that assigns adaptive weights to synthetic training data based on the model uncertainty, measured via the entropy of the model’s sample distribution for given questions. Specifically, with multiple sample predictions that LLM generated, EAST cluster them by final answer and measure the entropy value based on the cluster-based sample distribution. Then, EAST introduces a mapping function that transforms the entropy of model predictions into a bounded weight, under predefined constraints. This function includes a tunable parameter that controls the sharpness of the weighting, allowing flexible emphasis on uncertain data. By assigning higher weights to high-entropy data—those reflecting greater model uncertainty—EAST encourages the model to focus on more informative and challenging examples during training. Prioritizing such examples not only enhances reasoning capability but also helps prevent overfitting to overconfident data.

To address this gap, we introduce \textbf{E}ntropy-Based \textbf{A}daptive Weighting for \textbf{S}elf-\textbf{T}raining (EAST), a novel method that assigns adaptive weights to synthetic training data based on the model uncertainty, measured via the entropy of the model’s sample distribution for a given question. Specifically, EAST introduces a mapping function that transforms the entropy of model predictions into a bounded weight, under predefined constraints. This function includes a tunable parameter that controls the sharpness of the weighting, allowing flexible emphasis on uncertain examples. By assigning higher weights to high-entropy samples—those reflecting greater model uncertainty—EAST encourages the model to focus on more informative and challenging examples during training. Prioritizing such examples not only enhances reasoning capability but also helps prevent overfitting to overconfident data.

However, most self-training methodologies treat generated data uniformly, assigning equal importance to all generated samples. This approach fails to account for the varying educational value of different data points, which hinders the model’s ability to prioritize the most informative data and consequently limits the effectiveness of its learning process. This observation raises a natural question:

However, most self-training methodologies treat generated data uniformly, assigning equal importance to all generated samples. This approach fails to account for the varying educational value of different data points, which hinders the model’s ability to prioritize the most informative data and consequently limits the effectiveness of its learning process. This observation raises a natural question:

==> section/method2.tex <==


\section{Method}
In this section, we present Attention Preference Optimization (APO), a novel self-training strategy designed to maximize the utility of synthetic data generated by the self-training pipeline. APO prioritizes data based on both uncertainty and correctness, ensuring more effective learning. We first introduce the entropy-based and accuracy-based weighting components individually, followed by an explanation of how they are integrated into a unified objective. Figure~\ref{fig:apo} represents the general framework of APO. 

\subsection{Accuracy-Based Weight}
\label{sec:acc}
Traditional self-training methods assign equal weights to all data points during training, regardless of their impact on model improvement~\citep{zelikman2022star, singh2023beyond,chen2024self}. This uniform weighting disregards the model's existing knowledge and fails to emphasize areas requiring further refinement. For prompts or questions that the model already answers confidently and correctly, additional training on these samples provides minimal benefit and instead increases the risk of over-fitting to simpler data~\citep{huang2022large,singh2023beyond}. Effective self-training necessitates a focus on challenging examples, dynamically adjusting training emphasis based on model performance. 

To address this issue, we propose an accuracy-based weighting mechanism that prioritizes learning from data where the model exhibits lower performance, as these questions present greater challenges to the target model. Conversely, questions that consistently yield correct predictions receive lower emphasis during training, enhancing learning efficiency and reducing the risk of overfitting.

In the self-training pipeline, we generate $n$ samples for each question in the training data and compute the accuracy score based on the proportion of correct predictions:
\begin{equation}
A(x) = \frac{1}{n}\sum_{i=1}^{n} \mathbb{1}(y_i = y^*)
\end{equation}
where $y_i$ represents the i-th sampled prediction and $y^*$ denotes the ground truth. 
\subsubsection*{Mapping Function}

For notational simplicity, let $s_i = 1 - A(x_i)$ represent the inverse accuracy score for question $i$. Given a model's accuracy on each question, our goal is to transform these accuracy values into weights via a mapping function $f$, ensuring the following constraints:

\begin{equation}
\min(f(s)) \geq 0, \quad \frac{1}{N} \sum_{i=1}^{N} f(s_i) = 1.
\end{equation}

Let $\mu = \frac{1}{N} \sum_{i=1}^{N} s_i$ denote the mean of the set $\{s_i\}$. We consider three different mapping strategies:

\paragraph{(1) Simple Mean-Division Mapping}  
A straightforward approach is:

\begin{equation}
    f(s) = \frac{s}{\mu}
\end{equation}

which ensures that 

\begin{equation}
    \frac{1}{N} \sum_{i=1}^{N} f(s_i) = 1.
\end{equation}

However, this method lacks tunable parameters, offering no control over how the transformed values are distributed.

\paragraph{(2) Linear Transformation}  
To allow for control over the range of transformed values, we introduce a parameter $R$, representing the new range of mapped values. Defining the spreading ratio as $a = \frac{R}{\max(s) - \min(s)}$, we define the mapping function as:

\begin{equation}
    f(s) = a s + b, \quad a = \frac{R}{\max(s) - \min(s)}, \quad b = 1 - a \mu.
\end{equation}

Here, $a$ controls how the transformed values are spread, while $b$ is determined by the normalization constraint. Substituting $f(s)$ into the constraint:

$\frac{1}{N} \sum_{i=1}^{N} \bigl(a s_i + b\bigr) = a \mu + b = 1$, solving for $b$ gives $b = 1 - a \mu$.

To ensure non-negativity ($\min(f(s)) \geq 0$), we require:

\begin{equation}
    \min(f(s)) = a \min(s) + b = a (\min(s) - \mu) + 1 \geq 0.
\end{equation}

Rearranging, we obtain the constraint: $R \leq \frac{\max(s) - \min(s)}{\mu - \min(s)}.$ Thus, $R$ must be chosen within the range:

\begin{equation}
    R \in \Bigl(0, \frac{\max(s) - \min(s)}{\mu - \min(s)}\Bigr].
\end{equation}
\mandy{For range of R, it can go beyond this range if we allow the weight of 0 at some cases. We can introduce new threshold $\alpha$, for $s<\alpha$, s=0; $s>\alpha$, f(s) with $R>\frac{max(s)-min(s)}{\mu-min(s)}$.
\[
f(s) =
\begin{cases}
0, & s < \alpha,\\[4pt]
a\,s+b, & s \ge \alpha,\\[4pt]
\end{cases}
\]
}
While this linear approach adjusts the spread of values, it does not control the curvature of the transformation. That is, for $0 < a < 1$, the transformed values are compressed, whereas for $a > 1$, they are more dispersed. However, if the need to further emphasize certain value ranges differently (e.g., giving more attention to specific intervals), a nonlinear function is required.

\paragraph{(3) Non-Linear Transformation}  
 To control the curvature(``stretchness'') of the transformation, we define a non-linear mapping function:

\begin{equation}
    f(s) = c (s - s_0)^p + d.
\end{equation}

Here, $p$ determines the degree of stretching. By using the linear mapping function with parameter $R$, we control the new range of mapped value, allowing the shift of the mapping function. To study the impact of stretching on weighting, we first fix the new range of our data—eliminating any shifting—by setting $d=0$. This allows us to isolate the effect of a single hyperparameter, the stretch factor $p$. Since accuracy values start from 0 in our setting, we set $s_0 = 0$ without loss of generality, simplifying the function to:

\begin{equation}
    f(s) = c s^p.
\end{equation}

The constraint $\frac{1}{N} \sum_{i=1}^{N} f(s_i) = 1$ yields $c = \frac{N}{\sum_{i=1}^{N} s_i^p}$

thus:

\begin{equation}
    f(s) = s^p \cdot \frac{N}{\sum_{i=1}^{N} s_i^p} 
\end{equation}

Here, $p$ influences the curvature of the transformation:

\begin{equation}
    \begin{cases}
    p > 1   & \text{increases contrast (enhancing differences in weights)},\\
    0 < p < 1 & \text{reduces contrast (compressing differences)},\\
    p < 0   & \text{inverts the weight distribution (inverse stretching)}.
    \end{cases}
\end{equation}

Depending on the desired weight distribution, we can choose either the simpler linear mapping (which primarily affects spread) or the more flexible nonlinear transformation (which controls stretch and contrast).

Note: for linear function, we set $p=1$ and examine the effectness of how new range (how spread) the mapped value affect weighting; for non-linear function, we set $R$ as fixed and study the impact of stretchness on weighting.   
\subsubsection*{Mapping Function}

For notational simplicity, let $s_i = 1 - A(x_i)$ represent the inverse accuracy score for question $i$. Our goal is to map these accuracy values to weights via a function f in a way that more meaningfully captures near-perfect responses. However, raw accuracy alone often obscures these subtleties. We therefore require a transformation that (1) Monotonicity – Preserves the ranking of accuracy values while allowing for an increasing or decreasing trend.
(2) Curvature Control – Uses a parameter a to emphasize high-accuracy values by adjusting the shape of the transformation.
(3) Single-Parameter Parsimony – Depends on only one exponent a, simplifying both interpretation and tuning.

To fulfill these requirements, we adopt a power transformation of the form $y=x^a$, which is well-established in statistical modeling \citep{box1964analysis}. Finally, to normalize the transformed scores and avoid conflating overall learning progress with our weighting scheme, we impose the following constraint:  
\begin{equation}
\frac{1}{N} \sum_{i=1}^{N} f(s_i) = 1.
\end{equation}
This ensures that the average of the transformed values remains constant, allowing us to focus on how the chosen exponent a redistributes weights across different accuracy levels.
\subsubsection*{Threshold}

To prevent overly challenging prompts—those potentially beyond the model's current capabilities—from being assigned disproportionately high weights, we introduce a threshold \( t \). Specifically, if \( s > t \), we update the weight so that these examples do not have higher priority. We adopt two methods to update the weight:

(1) \textbf{Re-Weighting}  
For weights within the threshold, we simply set the reweighted value to 1 instead of assigning them a higher weight. This simultaneously increases the weight of examples where \( s \leq t \). The updated function is defined as:

\begin{equation}
\label{eq:acc}
\hat{f}(s) = 
\begin{cases}
1, & \text{if } s \ge t,\\
f(s), & \text{if } s < t.
\end{cases}
\end{equation}

With the introduction of \( t \), the hyperparameters \( R \) or \( p \) are adjusted accordingly. The two-segment function ensures that each segment is individually averaged to 1, preserving the previously established constraint. Thus, the mapping function \( f(s) \) continues to satisfy the required normalization condition.

(2) \textbf{Decreasing Function}  
For data within the threshold, re-weighting might cause a discontinuity in the function. To avoid this large jump, we introduce a decreasing function that gradually assigns less weight to extreme values. Since we enforce continuity between the two functions, for the mapping within the threshold \( s > t \) and letting \( N_t \) denote the number of examples within the threshold, we impose the following constraints:

\[
\min(f(s)) \geq 0, 
\quad \frac{1}{N_t} \sum_{i=1}^{N_t} f_t(s_i) = 1,
\quad f(t) = f_t(t).
\]

There are multiple types of decreasing functions that can be used. Similar to the mapping function, we adopt \( f(s) = c_t\,(s - s_0)^{p_t} + d \) as the decreasing function. Since we enforce \( f(t) = f_t(t) \), we set \( s_0 = t \) and \( d =  f(t) \) as the shifting parameters before applying the decreasing mapping function. The coefficient \( c \) is then determined by ensuring the average constraint is 1. Consequently, there are no free hyperparameters for the decreasing function. The decreasing function is defined as:
\[
f_t(s)
=
\begin{cases}
c_t\,(s-t)^{p_t}+f(t), & s\ge t,\\[4pt]
f(s), & s < t,
\end{cases}
\]

where $p_t$ is hyper-parameter and \[
  c_t\;=\;
  \frac{N(1-p)}
       {\sum_{i \in S_{t}} (s_i - t)^a}
  \,. 
\]


The final constraint is non-negativity. Since we introduce shifting, the decreasing function may result in negative values. To ensure non-negativity, if the decreasing mapping function yields negative values, we recalculate the scalar \( c_t \) with a more skewed value. At the same time, we introduce a new threshold \( \alpha \), where for \( s > \alpha \), the value is set to 0. Thus, when \( s < \alpha \), the decreasing function should have an average of 1, and for values larger than \( \alpha \), the function value is set to 0. The updated function is defined as:

\[
f_t(s) =
\begin{cases}
0, & s \ge \alpha,\\[4pt]
c_t\,(s-t)^{p_t}+f(t), & t < s \le \alpha,\\[4pt]
f(s), & s < t.
\end{cases}
\]

In practice, there is no closed-form solution for calculating \( \alpha \); therefore, we determine it using the bisection method as described below.
 
\input{section/threshold}


% \begin{equation}
% \label{eq:acc}
% \hat{f}(s) = 
% \begin{cases}
% a_{t}s+b_t, & \text{if }s \ge t,\\
% f(s), & \text{if } s < t,
% \end{cases}
% \end{equation}
% Now to calculate the value of $a$ and $b$, we assume $a_t*t+b_t=p=f(t)$ where $p$ is obtained from mapping function, then we will have functions $a_t*t+b_t=p$ and $\frac{1}{N_t}\sum_{i=1}^{N_t} f_t(s_i)=a_t*\mu_t+b=1$, from there we solved the function and get $a=$ and $b=$, where $a=\frac{1-p}{\mu_t-t}$ and $b=\frac{p*\mu_t-t}{\mu_t-t}$ are calculated based on constraints, no additional hypaperameter are added. However, this may not ensure the non-negativity of the mapped value. to ensure the non-negativity, we need to introduce a new point $\alpha$, if value larger than $\alpha$, set it to 0, otherwise set it to the decreasing mapping function. 
% \[
% f_t(s)
% =
% \begin{cases}
% 0, & s \ge \alpha,\\[4pt]
% a\,s + b, & t < s \le \alpha,\\[4pt]
% f(s), & s < t,
% \end{cases}
% \]
% \textbf{(3) Non-linear decreasing function}. Similar to previous section, since if we want to change the stretchness of the decreasing funcito,  we may use different non-linear function, as followed


\subsection{Entropy-Based Weight}
Many studies have found that large language models (LLMs) tend to be resistant to changing their predictions, particularly when they are highly confident in their responses~\citep{kumar2024training, yang2024confidence, li2024confidence}. Therefore, guiding the model to focus on areas where it lacks confidence or is uncertain becomes a natural next step. Research indicates that prioritizing learning from uncertain questions—rather than those where the model is stubborn—leads to a more effective learning process~\citep{kumar2024training, li2024confidence}.

Previous studies indicate that introducing an entropy component into the training objective can benefit model training~\citep{omura2024entropy, zhang2024entropy}. Following this intuition, we introduce an entropy-based approach that encourages models to focus on learning from the most uncertain data. The core insight is that questions with higher entropy values indicate greater model uncertainty, meaning the model lacks a strong preference among possible answers. Prioritizing such questions during training requires smaller parameter updates, facilitating convergence to correct solutions. 

In the self-training pipeline, we generate $n$ samples for each question and cluster them into $k$ groups ($k \leq n$) based on their final answers, where each cluster represents a distinct answer. The underlying assumption is that samples culminating in the same final answer follow similar reasoning patterns. Therefore, each group represents the model's inherent preference for specific reasoning paths. When the number of sparse groups ($k$) is higher, it indicates greater model uncertainty for a question, while a distribution concentrated around a single reasoning path suggests higher confidence. The model's uncertainty for a given question is quantified through the entropy value, which is calculated based on the $k$ clusters using:
\begin{equation}
H = -\sum_{i=1}^{k} p_i \log p_i
\end{equation}
where $p_i$ represents the proportion of samples in cluster $i$ relative to the total number of samples.
Similar to the accuracy-based approach, we apply a linear transformation $g(x) = ax + b$ with threshold $t$, where $a, b, t$ are hyperparameters. 
\begin{equation}
\label{eq:entropy}
f(\hat{H}(x)) = 
\begin{cases}
1, & \text{if } A(x) \leq t,\\
a \cdot \text{H(x)} + b, & \text{if } A(x) > t,
\end{cases}
\end{equation}

This transformation is constrained such that the average entropy across the training dataset equals 1:
\begin{equation}
\frac{1}{|D|}\sum_{x \in D} f(\hat{H}(x)) = 1
\end{equation}
where $D$ represents the training dataset and $H(x)$ denotes the entropy value for sample $x$.

\subsection{Combined Objective}
The final weighting objective combines accuracy-based and entropy-based values using a mixing parameter $\alpha \in [0,1]$:
\begin{equation}
w(x) = \alpha f(\hat{H}(x)) + (1-\alpha)g(\hat{A}(x))
\end{equation}
where $f(\hat{H}(x))$ represents the transformed entropy-based value and $g(\hat{A}(x))$ represents the transformed accuracy-based value. This combined weighting strategy enables a balanced influence of uncertainty and correctness during training. 

This weighting is then incorporated into the alignment loss objective as:
\begin{equation}
\label{eq:w}
    \mathcal{L}_{\mathrm{APO_{DPO}}}(\theta,\theta_{\mathrm{ref}}) = w * \mathcal{L}_{\mathrm{DPO}}(\theta,\theta_{\mathrm{ref}})
\end{equation}
Moreover, APO is flexible and can be adapted to incorporate other loss functions. 





==> section/threshold.tex <==

% \section*{Piecewise Linear Function with Clamping to Ensure Nonnegativity}

% The goal is to define a piecewise linear mapping that:
% \begin{itemize}
%     \item Remains continuous at a threshold \(t\) where the mapping must match an existing function \(f(t)\).
%     \item Maintains an average value of 1 for data points \(s_i \le t\).
%     \item Ensures that the mapped values never go below 0.
% \end{itemize}

% \noindent
% We achieve this by introducing a two-segment function:
% \[
% f_t(s) \;=\;
% \begin{cases}
% 0, & s \ge \alpha,\\[6pt]
% a\,s + b, & t < s \le \alpha,\\[6pt]
% f(s), & s < t,
% \end{cases}
% \]
% .

% \subsection*{Step 1: Impose Continuity at \(\boldsymbol{s = t}\)}

% Let \(p = f(t)\). We require
% \[
% a\,t + b \;=\; p.
% \tag{1}
% \]
% This ensures that the piecewise linear segment connects smoothly with the outside function \(f(s)\) at \(s = t\).

% \subsection*{Step 2: Impose Nonnegativity by Anchoring at \(\boldsymbol{\alpha}\)}

% We set \(f_t(\alpha) = 0\). Hence,
% \[
% a\,\alpha + b \;=\; 0.
% \]
% From Eq.~\eqref{(1)} we have \(b = p - a\,t\). Therefore,
% \[
% a\,\alpha + (p - a\,t) \;=\; 0
% \quad\Longrightarrow\quad
% a\,(\alpha - t) \;=\; -p
% \quad\Longrightarrow\quad
% a \;=\; -\,\frac{p}{\,\alpha - t\,}.
% \tag{2}
% \]
% Substituting back into \(b = p - a\,t\),
% \[
% b 
% = p - \Bigl(-\frac{p}{\,\alpha - t\,}\Bigr)\,t
% = p + \frac{p\,t}{\,\alpha - t\,}
% = p\,\frac{\alpha}{\,\alpha - t\,}.
% \tag{3}
% \]
% Thus, for \(t < s \le \alpha\),
% \[
% f_t(s)
% \;=\;
% -\frac{p}{\,\alpha - t\,}\,s
% \;+\;
% p\,\frac{\alpha}{\,\alpha - t\,}.
% \]

% \subsection*{Step 3: Impose the Average-Weight Constraint}

% Let \(N_t\) be the number of data points \(\{s_i \mid s_i \ge t\}\). We require
% \[
% \frac{1}{N_t}\,\sum_{i=1}^{N_t} f_t(s_i) \;=\; 1.
% \]
% Define the sets
% \[
% S_{1} = \{\,s_i : s_i \ge \alpha\}, \quad
% S_{2} = \{\,s_i : t < s_i \le \alpha\}.
% \]
% For \(s_i \in S_{1}\), \(f_t(s_i) = 0\). For \(s_i \in S_{2}\),
% \(\displaystyle f_t(s_i) = a\,s_i + b\). Therefore,
% \[
% \sum_{i=1}^{N_t} f_t(s_i) 
% \;=\;
% \sum_{s_i \in S_{1}} 0
% \;+\;
% \sum_{s_i \in S_{2}} \bigl(a\,s_i + b\bigr)
% \;=\;
% a\,\sum_{s_i \in S_{2}} s_i
% \;+\;
% b\,\lvert S_{2}\rvert.
% \]
% Hence,
% \[
% \frac{1}{N_t}\Bigl[a\,\sum_{s_i \in S_{2}} s_i + b\,\lvert S_{2}\rvert\Bigr]
% \;=\;
% 1.
% \tag{4}
% \]
% Substitute \(a\) and \(b\) from Eqs.~\eqref{(2)}--\eqref{(3)}:
% \[
% a = -\,\frac{p}{\,\alpha - t\,},
% \quad
% b = p\,\frac{\alpha}{\,\alpha - t\,}.
% \]
% Then,
% \[
% \sum_{s_i \in S_{2}} (a\,s_i + b)
% = 
% \sum_{s_i \in S_{2}}
% \Bigl[
% -\frac{p}{\,\alpha - t\,}\,s_i 
% \;+\; 
% p\,\frac{\alpha}{\,\alpha - t\,}
% \Bigr]
% =
% \frac{p}{\,\alpha - t\,}
% \sum_{s_i \in S_{2}} (\alpha - s_i).
% \]
% Thus Eq.~\eqref{(4)} becomes
% \[
% \frac{1}{N_t}
% \cdot
% \frac{p}{\,\alpha - t\,}
% \sum_{s_i \in S_{2}} (\alpha - s_i)
% \;=\;
% 1
% \quad\Longrightarrow\quad
% p
% \;=\;
% \frac{N_t \, (\alpha - t)}{\sum_{s_i \in S_{2}} (\alpha - s_i)}.
% \tag{5}
% \]

% \subsection*{Finding \(\boldsymbol{\alpha}\) Numerically}

% Because the set \(S_{2}\) depends on \(\alpha\) (i.e., which points lie above \(\alpha\)), Eq.~\eqref{(5)} generally requires a numerical solution:
% \begin{enumerate}
%     \item \emph{Guess} a value for \(\alpha\).
%     \item Determine which points \(s_i\) lie in \(S_{2}\).
%     \item Compute the right-hand side of Eq.~\eqref{(5)} and compare to \(p\).
%     \item Adjust \(\alpha\) (e.g., using bisection or another root-finding method) until both sides match.
% \end{enumerate}
% Once \(\alpha\) is obtained, one can directly compute \(a\) and \(b\) from Eqs.~\eqref{(2)}--\eqref{(3)}.

% \subsection*{Final Piecewise-Linear+Clamping Function}

% After determining \(\alpha\) via the above steps:
% \[
% f_t(s)
% =
% \begin{cases}
% 0, & s \ge \alpha,\\[4pt]
% a\,s + b, & t < s \le \alpha,\\[4pt]
% f(s), & s < t,
% \end{cases}
% \]
% with
% \[
% a = -\,\frac{p}{\,\alpha - t\,}
% \quad\text{and}\quad
% b = p\,\frac{\alpha}{\,\alpha - t\,}.
% \]
% This approach guarantees:
% \begin{itemize}
%     \item \(\min f_t(s) \ge 0\).
%     \item Continuity at \(s = t\) (i.e., \(f_t(t) = f(t)\)).
%     \item An average value of 1 for \(\{ s_i \mid s_i \ge t\}\).
% \end{itemize}



% \section*{Constructing \(\boldsymbol{f(s) = s^a e^b}\) Under Two Constraints}

% We wish to find parameters \(a\) and \(b\) so that
% \[
% f(s) \;=\; e^{\,a \ln(s) + b} \;=\; s^a \, e^b
% \]
% satisfies the following conditions:
% \begin{enumerate}
% \item \(\displaystyle f(t) \;=\; p.\)
% \item \(\displaystyle \frac{1}{N}\sum_{i=1}^N f(s_i) \;=\; 1,\) where \(\{s_1, \ldots, s_N\}\) is a given set of positive data points.
% \end{enumerate}

% \subsection*{1. Functional Form and Constraints}

% We have
% \[
% f(s) \;=\; s^a \, e^b,
% \]
% with unknowns \(a\) and \(b\). The two constraints become:

% \begin{enumerate}
% \item \textbf{Match at \(s = t\):}
% \[
% f(t) \;=\; t^a\,e^b \;=\; p.
% \tag{1}
% \]
% \item \textbf{Average equals 1:}
% \[
% \frac{1}{N}\sum_{i=1}^N f(s_i)
% \;=\;
% \frac{1}{N}\sum_{i=1}^N \bigl(s_i^a\, e^b\bigr)
% \;=\;
% e^b\,\frac{1}{N}\sum_{i=1}^N s_i^a
% \;=\;
% 1.
% \tag{2}
% \]
% \end{enumerate}

% \subsection*{2. Solving for \(\boldsymbol{a}\) and \(\boldsymbol{b}\)}

% From Eq.~\eqref{(2)}:
% \[
% e^b
% \;=\;
% \frac{1}{\frac{1}{N}\sum_{i=1}^N s_i^a}
% \;=\;
% \frac{N}{\sum_{i=1}^N s_i^a}.
% \tag{2'}
% \]
% Substitute this into Eq.~\eqref{(1)}:
% \[
% t^a\,\left(\frac{N}{\sum_{i=1}^N s_i^a}\right)
% \;=\;
% p
% \quad\Longrightarrow\quad
% p\,\sum_{i=1}^N s_i^a
% \;=\;
% N \, t^a.
% \]
% Rearrange:
% \[
% \sum_{i=1}^N s_i^a
% \;=\;
% \frac{N\,t^a}{p}.
% \tag{3}
% \]
% Define the function
% \[
% \Phi(a)
% \;=\;
% \sum_{i=1}^N \bigl(s_i^a\bigr)
% \;-\;
% \frac{N\,t^a}{p}.
% \]
% We want to solve
% \[
% \Phi(a) \;=\; 0
% \]
% for \(a\). Generally, this has no closed-form solution, so we use a numerical root-finding method (e.g., bisection, Newton, or secant).

% \subsection*{3. Numerical Procedure for \(\boldsymbol{a}\)}

% \begin{enumerate}
% \item \emph{Initialize} with a bracket or guess for \(a\), say \(a_{\text{low}}\) and \(a_{\text{high}}\).
% \item \emph{Evaluate} \(\Phi(a_{\text{low}})\) and \(\Phi(a_{\text{high}})\). Ensure they have opposite signs (if possible).
% \item \emph{Iterate} using bisection (or another method) until \(\Phi(a)\) is sufficiently close to 0.
% \item The final converged \(a\) solves \(\Phi(a)=0\).
% \end{enumerate}

% \subsection*{4. Once \(\boldsymbol{a}\) is Found, Solve for \(\boldsymbol{b}\)}

% From Eq.~\eqref{(2')}:
% \[
% e^b
% \;=\;
% \frac{N}{\sum_{i=1}^N s_i^a}
% \quad\Longrightarrow\quad
% b
% \;=\;
% \ln\!\bigl(N\bigr)
% \;-\;
% \ln\Bigl(\sum_{i=1}^N s_i^a\Bigr).
% \]

% \subsection*{5. Final Function}

% Plug the found values of \(a\) and \(b\) into
% \[
% f(s)
% \;=\;
% s^a \, e^b.
% \]
% This guarantees
% \begin{itemize}
% \item \(\displaystyle f(t) = p\).
% \item \(\displaystyle \frac{1}{N}\sum_{i=1}^N f(s_i) = 1.\)
% \end{itemize}

% \subsection*{6. Summary of Steps}

% \begin{enumerate}
% \item Propose \(f(s) = s^a e^b\).
% \item Impose \(f(t)=p \implies t^a e^b=p\).
% \item Impose \(\frac{1}{N}\sum f(s_i)=1 \implies e^b \frac{1}{N}\sum s_i^a=1\).
% \item Combine to get \(p\sum s_i^a = N t^a\), leading to
% \[
% \Phi(a) \;=\; \sum_{i=1}^N s_i^a - \frac{N\,t^a}{p} = 0.
% \]
% \item Solve \(\Phi(a)=0\) numerically for \(a\).
% \item Compute \(b = \ln(N) - \ln(\sum_{i=1}^N s_i^a)\).
% \item Final mapping: \(f(s) = s^a e^b\).
% \end{enumerate}


% % \section{(3) Non-Linear Transformation.}  
% \mandy{s=s-min, otherwise we need some further shift?}
%     To control the strechness of the function we define new non-linear function as:
%     \[
%     f(s) = e^{\,a \ln(s) + b} \;=\; s^a \, e^b.
%     \]
%     We must satisfy the constraint:
%     \[
%     \frac{1}{N}\sum_{i=1}^{N} f(s_i) = 1 \quad \Longrightarrow \quad
%     \frac{1}{N}\sum_{i=1}^{N} s_i^a \, e^b = 1.
%     \]
%     Solving for \(b\) gives:
%     \[
%     b = \ln\Bigl(\frac{N}{\sum_{i=1}^{N} s_i^a}\Bigr),
%     \]
%     thus:
%     \[
%     f(s) = s^a \; \frac{N}{\sum_{i=1}^{N} s_i^a} = s^{\frac{R}{max(s)-min(s)}} \; \frac{N}{\sum_{i=1}^{N} s_i^{\frac{R}{max(x)-min(x)}}}.
%     \]
%     Here, \(a\) (analogous to \(R\) in the linear case) adjusts the spread:
%     \[
%     \begin{cases}
%     a > 1   & \text{increases the contrast (larger stretch)},\\
%     0 < a < 1 & \text{reduces the contrast (smaller stretch)},\\
%     a < 0   & \text{inverts the relationship (inverse stretch)}.
%     \end{cases}
%     \]
%     Depending on how widely we want to distribute the weights, we can choose either
%     the simpler linear form controlled by \(R\) or the more flexible non-linear form
%     controlled by \(a\).



\subsubsection*{Piecewise-Linear Model with Cutoff \(\alpha\)}

% We define
% \[
%   f(s)
%   \;=\;
%   \begin{cases}
%     (\,s - t\,)^{a}\,b \;+\; p, & \text{if } s < \alpha, \\[6pt]
%     0, & \text{if } s \ge \alpha,
%   \end{cases}
% \]
% where \(t\) and \(p\) are fixed, \(a\) may be treated as a hyperparameter (or solved for), and \(\alpha\) is a ``cutoff'' that forces \(f\) to vanish for \(s \ge \alpha\).  The scalar \(b\) is chosen (for given \(a, \alpha\)) so that the \emph{average} of \(f\) over data points is 1, while maintaining \(f(t)=p\) automatically if \(t<\alpha\).

% \subsection*{1. Automatic Constraint \(f(t)=p\)}

% Observe that
% \[
%   f(t)
%   \;=\;
%   (\,t - t\,)^{a}\,b \;+\; p
%   \;=\;
%   p.
% \]
% Hence \(f(t)=p\) holds for any \(a, b\) \emph{whenever} \(t < \alpha\).  If \(t \ge \alpha\), then \(f(t)=0\), which conflicts with wanting \(f(t)=p\).  Thus we usually assume \(t < \alpha\).

% \subsection*{2. Imposing the Mean = 1 Condition}

Let \(\{\,s_1,\dots,s_N\}\) be our data points.  We require $\frac{1}{N} \sum_{i=1}^N f(s_i)
  \;=\;
  1.$
Define $S_{\alpha}
  \;=\;
  \bigl\{\, i \,\bigm|\; s_i < \alpha \bigr\}.$, and $f(t)=k$
Then
\[
  \sum_{i=1}^N f(s_i)
  \;=\;
  \sum_{i \in S_{\alpha}} \Bigl((s_i - t)^{p_t}\,c_t + k\Bigr) 
  \;+\;
  \sum_{i \notin S_{\alpha}} 0
  \;=\;
  c_t \sum_{i \in S_{\alpha}} (s_i - t)^{p_t} \;+\; k\,\bigl|S_{\alpha}\bigr|.
\]
We want \(\tfrac{1}{N}\) times this sum to be 1, so
\[
  c_t \sum_{i \in S_{\alpha}} (s_i - t)^{p_t} \;+\; k\,\bigl|S_{\alpha}\bigr|
  \;=\;
  N.
\]
Hence we can solve for \(c_t\):
\[
  c_t
  \;=\;
  \frac{\,N \;-\; k\,\bigl|S_{\alpha}\bigr|\,}
       {\sum_{i \in S_{\alpha}} (s_i - t)^{p_t}}
  \,.
\]
Crucially, \(c_t\) may be negative, zero, or positive.  

\subsection*{Ensuring \(f\ge0\)}

If we want \(f(s)\ge0\) for all \(s\):

\begin{itemize}
\item For \(s_i \ge \alpha\), we have \(f(s_i)=0\), already nonnegative.
\item For \(s_i < \alpha\), we need
  \[
    (s_i - t)^{p_t}\,c_t \;+\; p
    \;\ge\;
    0.
  \]
  Once \(b\) is determined from the mean=1 formula, one checks whether any of those values is negative.  If some are negative, one can adjust \(\alpha\) to remove the offending points from the ``power-law region'' (i.e.\ ensure they satisfy \(s_i \ge \alpha\)).
\end{itemize}

\subsection*{Summarized Algorithmic Steps}

\begin{enumerate}
\item \textbf{Sort} the data \(\{s_i\}\) (optional but helpful).
\item \textbf{Pick or bracket} values for \(\alpha\).
\item For each \(\alpha\):
  \begin{enumerate}
    \item Identify the subset \(S_{\alpha}=\{\,i\mid s_i<\alpha\}\).
    \item Solve
      \[
        c_t
        \;=\;
        \frac{\,N - k\,|S_{\alpha}|\,}
             {\sum_{\,i\in S_{\alpha}} (s_i - t)^{p_t}}
      \]
      for \(c_t\), provided the denominator is not zero.
    \item Check positivity of \(\bigl((s_i - t)^{p_t}\,c_t + k\bigr)\) for \(s_i<\alpha\).  If any is negative, that choice of \(\alpha\) fails.
    \item Compute the mean of \(f(s_i)\).  If it equals 1 (within tolerance), record \(\alpha\) as a valid solution. Otherwise, adjust \(\alpha\) (e.g.\ via bisection).
  \end{enumerate}
\end{enumerate}

\noindent
In this way, we can systematically find a piecewise function
\[
  f(s)
  \;=\;
  \begin{cases}
    (s - t)^{p_t}\,c_t + k, & s<\alpha,\\
    0, & s\ge\alpha,
  \end{cases}
\]
that (1) has sample mean 1, (2) never goes negative, and (3) has \(f(t)=k\).  




==> table/main_exp2.tex <==

% \begin{table*}[t]
% \caption{Experimental results on GSM8K and MATH benchmark. The best performing score is highlighted in \textbf{bold}. \wei{I do not see any bold scores. Also what are the two color bands below the table?}}
% \label{table:main}
% \centering
% % \small
% % \setlength{\tabcolsep}{4pt}
% \resizebox{0.99\textwidth}{!}{% 
% \begin{tabular}{lcccccc}  % Changed first column to left-aligned
% \toprule
% \multirow{2}{*}{Setting} 
% & \multicolumn{3}{c}{\texttt{LLaMA-3.2-1B}} & \multicolumn{3}{c}{\texttt{LLaMA-3.1-8B}} \\
% & GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ & GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ \\
% \midrule
% \textit{default} & 46.2& 28.5& 37.3& 82.8& 50.4&66.6\\
% \hline
% % \textit{default} & 37.23& 25.50& 31.37 & & & \\
% SFT & 50.1& 28.4& 39.2&85.0 & 50.0&67.5\\
% Perplexity & 50.9&28.5 & 39.7& 84.8&50.9 &67.8\\
% EAST & 51.8& 29.4& 40.6& 86.1&51.2 &68.6\\
% \hline
% DPO & 50.2&28.7 & 39.5& 84.6& 50.5& 67.5\\
% Perplexity* &  50.9& 28.1& 39.5& 85.1&50.2 & 67.6\\
% EAST & 51.9& 29.7& 40.8& 85.4& 50.9& 68.1\\
% % \hline

% % KTO & & & & & & \\
% % Perplexity & & & & & & \\
% % APO & & & & & & \\

% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% % \vspace{-5em}
% \caption{Experimental results on GSM8K and MATH benchmark.  }
% \label{table:main}
% \centering
% \SetTblrInner{rowsep=0.95pt}
% \begin{tblr}{
%   colspec = {ccccccc},
%   row{1-2} = {bg=gray!25},        % Header rows background
%   row{4-6, 10-12} = {bg=gray!10},    % Highlight SFT row
%   % hlines,
%   % vlines,
% }
% \toprule
% \SetCell[r=2]{c}{Setting} & \SetCell[c=3]{c}{\texttt{LLaMA-3.2-1B}} & & &   \SetCell[c=3]{c}{\texttt{LLaMA-3.2-1B}} & &   \\
% % \SetCell[r=2]{c}{Setting} & \SetCell[c=3]{c}\texttt{LLaMA-3.2-1B} & \\
% % \SetCell[c=3]{c}\texttt{LLaMA-3.1-8B} \\
% \cmidrule[lr]{2-4}\cmidrule[lr]{5-7}
% & GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ & GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ \\
% \midrule
% \textit{default} & 46.2 & 28.5 & 37.3 & 82.8 & 50.4 & 66.6 \\
% SFT              & 50.1 & 28.4 & 39.2 & 85.0 & 50.0 & 67.5 \\
% Perplexity       & 50.9 & 28.5 & 39.7 & 84.8 & 50.9 & 67.8 \\
% EAST             & 51.8 & 29.4 & 40.6 & 86.1 & 51.2 & 68.6 \\
% DPO              & 50.2 & 28.7 & 39.5 & 84.6 & 50.5 & 67.5 \\
% Perplexity*      & 50.9 & 28.1 & 39.5 & 85.1 & 50.2 & 67.6 \\
% EAST             & 51.9 & 29.7 & 40.8 & 85.4 & 50.9 & 68.1 \\

% KTO              & 50.2 & 28.7 & 39.5 & 84.6 & 50.5 & 67.5 \\
% Perplexity*      & 50.9 & 28.1 & 39.5 & 85.1 & 50.2 & 67.6 \\
% EAST             & 51.9 & 29.7 & 40.8 & 85.4 & 50.9 & 68.1 \\
% \bottomrule
% \end{tblr}
% % \end{table*}

\begin{table*}[t]
\caption{Experimental results on GSM8K and MATH benchmark. The best performance across the vanilla loss function and its three weighting strategies is highlighted in \textbf{bold}. Significant boost ($\ge$ 1\%) over both the vanilla method and baselines are \underline{underlined}.}
\label{table:main}
\centering
\SetTblrInner{rowsep=0.95pt}
\resizebox{0.98\textwidth}{!}{%
\begin{tblr}{
  colspec = {lcccccc},
  row{1-2} = {bg=gray!25},        
  row{4-7, 12-15} = {bg=gray!10},  
}
\toprule
\SetCell[r=2]{l}{Setting} & \SetCell[c=3]{c}{\texttt{LLaMA-3.2-1B}} & & & \SetCell[c=3]{c}{\texttt{LLaMA-3.1-8B}} & & \\
\cmidrule[lr]{2-4}\cmidrule[lr]{5-7}
& GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ & GSM8K$(\%)$ & MATH$(\%)$ & AVG$(\%)$ \\
% & GSM8K(\%) & MATH(\%) & AVG(\%) & GSM8K(\%) & MATH(\%) & AVG(\%) \\
\midrule
\textit{default} & 46.2 & 28.5 & 37.3 & 82.8 & 50.4 & 66.6 \\
SFT              & 50.1 & 28.4 & 39.2 & 85.0 & 50.0 & 67.5 \\
+\textit{LW}       & 50.9 & 28.5 & 39.7 & 84.8 & 50.9 & 67.8 \\
+\textit{LW(P)}       & 51.2& 28.4&  39.8&  85.1&  50.8& 68.0 \\
+\textit{EAST  }           & \textbf{51.8} & \textbf{29.4} & \textbf{40.6} & \underline{\textbf{86.1}} & \textbf{51.2} & \textbf{68.6} \\
\textit{DPO}              & 50.2 & 28.7 & 39.5 & 84.6 & 50.5 & 67.5 \\
+LW      & 50.9 & 28.1 & 39.5 & 85.1 & 50.2 & 67.6 \\
+LW(P)       & 50.3&28.4& 39.4 & 85.1 &  50.8& 68.0 \\
+EAST             & \underline{\textbf{51.9}} & \underline{\textbf{29.7}} & \underline{\textbf{40.8}} & \textbf{85.4} & \textbf{50.9} & \textbf{68.1} \\
KTO              & 53.0 & 28.8 & 40.9 & 83.9 & 48.9 & 66.4 \\
+LW      & 52.9 & 28.2 & 40.6 &  84.3&  49.1&  66.7\\
+LW(P)       & 52.9& 28.9& 40.9 & 83.9 & 49.1 & 66.5 \\
+EAST             & 53.0 & 29.9 &  &  85.1&  51.0&  \\
\bottomrule
\end{tblr}%
}
\end{table*}



